CoMBO: Conflict Mitigation via Branched Optimization for Class Incremental Segmentation

Effective Class Incremental Segmentation (CIS) requires simultaneously mitigating catastrophic forgetting and ensuring sufficient plasticity to integrate new classes. The inherent conflict above often leads to a back-and-forth, which turns the objective into finding the balance between the performance of previous~(old) and incremental~(new) classes. To address this conflict, we introduce a novel approach, Conflict Mitigation via Branched Optimization~(CoMBO). Within this approach, we present the Query Conflict Reduction module, designed to explicitly refine queries for new classes through lightweight, class-specific adapters. This module provides an additional branch for the acquisition of new classes while preserving the original queries for distillation. Moreover, we develop two strategies to further mitigate the conflict following the branched structure, \textit{i.e.}, the Half-Learning Half-Distillation~(HDHL) over classification probabilities, and the Importance-Based Knowledge Distillation~(IKD) over query features. HDHL selectively engages in learning for classification probabilities of queries that match the ground truth of new classes, while aligning unmatched ones to the corresponding old probabilities, thus ensuring retention of old knowledge while absorbing new classes via learning negative samples. Meanwhile, IKD assesses the importance of queries based on their matching degree to old classes, prioritizing the distillation of important features and allowing less critical features to evolve. Extensive experiments in Class Incremental Panoptic and Semantic Segmentation settings have demonstrated the superior performance of CoMBO. Project page: https://guangyu-ryan.github.io/CoMBO.

==> sec/0_abstract.tex <==
\begin{abstract}
Effective Class Incremental Segmentation (CIS) requires simultaneously mitigating catastrophic forgetting and ensuring sufficient plasticity to integrate new classes. 
The inherent conflict above often leads to a back-and-forth, which turns the objective into finding the balance between the performance of previous~(old) and incremental~(new) classes.
To address this conflict, we introduce a novel approach, Conflict Mitigation via Branched Optimization~(CoMBO).
Within this approach, we present the Query Conflict Reduction module, designed to explicitly refine queries for new classes through lightweight, class-specific adapters.
% This module facilitates a branched way to knowledge acquisition, diverging from traditional knowledge distillation for old classes.
This module provides an additional branch for acquisition of new classes while preserves the original queries for distillation. 
% Following the branched structure, 
% we have developed two knowledge distillation strategies that are integrated within the Mask2Former architecture to further mitigate the conflict, 
Moreover, we develop two strategies to further mitigate the conflict following the branched structure, 
i.e., the Half-Learning Half-Distillation~(HDHL) over classification probabilities, and the Importance-Based Knowledge Distillation~(IKD) over query features.
HDHL selectively engages in learning for classification probabilities of queries that match the ground truth of new classes, while aligning unmatched ones to the corresponding old probabilities, thus ensuring retention of old knowledge while absorbing new classes via learning negative samples.
Meanwhile, IKD assesses the importance of queries based on their matching degree to old classes, prioritizing the distillation of important features and allowing less critical features to evolve.
Extensive experiments in Class Incremental Panoptic and Semantic Segmentation settings have demonstrated the superior performance of CoMBO. 
The code is available at \url{https://github.com/KaiXu47/CoMBO}.
\end{abstract}

% To address this conflict, we introduce a Harmonious Acquisition and Retention Method for Old and New Yield (HARMONY). 
% , which incorporates three novel knowledge distillation mechanisms within the widely used Mask2Former architecture.

% refined features to promote preserving original unrefined features while. 
% HDHL strategy selectively applies distillation to unmatched~(non-object) masks and classification learning to matched masks.
% Furthermore, our Query Conflict Reduction module enables refining queries for new classes using class-specific adapters before distillation, thereby maintaining original features while promoting seamless class integration.

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figs/start.png}
    \caption{Brief comparison of our improved distillation and learning strategy (below) and previous conflicting distillation and learning strategies (above). 
    The previous strategy acts contradictory supervision on the same target for finding the balance point, while our strategy, including the importance factor for distillation and the QCR module for adaptive learning, constructs more compatible separated supervision on different targets. 
    The visualization result on the incremental classes (`\textit{Traffic Light}') demonstrates the effectiveness of our strategy. }
    \label{fig:brief}
\end{figure}

Semantic segmentation, the fundamental task in computer vision, involves classifying each pixel into predefined categories.
Panoptic segmentation, the challenging variant, unifies semantic and instance segmentation to both classify every pixel and simultaneously identify distinct object instances.
Recent advancements in mask classification-based segmentation, such as MaskFormer~\cite{maskformer} and Mask2Former~\cite{mask2former}, enable the unification of semantic and panoptic segmentation.
However, traditional approaches to segmentation suffer from limitations in dynamic environments where new classes can emerge unpredictably, as they are typically trained on a static set of categories.
Therefore, Class Incremental Segmentation (CIS) has emerged as a pivotal task for continually learning new categories, where models can adapt to new classes without forgetting previously learned ones.

Historically, studies in Class Incremental Semantic Segmentation~(CISS)~\cite{alife22,dkd22,coinseg23} mainly focuses on tackling \textit{catastrophic forgetting}, employing various techniques such as knowledge distillation~\cite{mib20,plop21,rcil22}, freezing parameters~\cite{ssul21,micro22,eclipse24}, or generating pseudo-labels from old model~\cite{plop21}. 
More recent efforts~\cite{comformer23,balconpas24} 
have extended these techniques to the more challenging Class Incremental Panoptic Segmentation~(CIPS) based on the advanced Mask2Former.
Nonetheless, these methods often fail to adequately reconcile the inherent tension between retaining old knowledge and acquiring new information.
% However, these methods often struggle to find a balance between the conflicting goals of acquisition and retention.
Some overemphasize maintaining stability, thus hindering the learning of new classes, while others prioritize plasticity, leading to significant forgetting of old classes. 
% Both these two types of methods ignore jumping out of the constraint to reduce conflicts. 
It is necessary to deconstruct these conflicting objectives to facilitate a more compatible incremental learning process, achieving promotion in both the acquisition of new classes and retention of old classes.

In this work, we introduce the Conflict Mitigation via Branched Optimization~(CoMBO), to reduce the conflicts between the acquisition of new classes and the retention of old classes.
By integrating three specialized knowledge distillation mechanisms within the Mask2Former architecture, CoMBO effectively mitigates catastrophic forgetting while enhancing the model's ability to assimilate new classes.
Using bipartite matching, Mask2Former optimally aligns each query, complete with its classification logits and mask predictions, with the most fitting ground truth class, ensuring efficient optimization.
% Mask2Former utilizes bipartite matching to optimally pair each query, which includes corresponding classification logits and mask predictions, with the most appropriate ground truth class for effective optimization.
Therefore, we first introduce the Half-Learning Half-Distillation mechanism, which selectively applies a shared Kullback-Leibler divergence to the classification logits of unmatched queries.
This method distinctly separates the distillation on unmatched masks from the classification optimization of matched ones.
% \gao{This approach distills the logits from old classes with distillation loss while optimizing the logits for new classes with classification loss.}
Moreover, unlike traditional methods that apply uniform distillation to all features, we introduce an importance-based knowledge distillation technique. 
This technique assesses the significance of each query in preserving knowledge about old classes and adjusts the distillation intensity accordingly, emphasizing the retention of key queries.
Additionally, our Query Conflict Reduction module innovatively adapts features for new classes while maintaining the queries' original characteristics before distillation, using class-specific adapters for each newly learned class.
% Additionally, a Query Conflict Reducing module is proposed to separately adapt features for learning new classes while preserving the original characteristics of the queries. 
% This module incorporates class-specific adapters for each newly learned class.
Finally, our approach outperforms previous methods in multiple benchmarks, especially in typical and challenging scenarios such as 100-10 of ADE20K. 
Our approach achieves remarkable performance of 35.6\% and 41.1\% mIoU on 100-10 of CIPS and CISS, respectively, compared to the previous state-of-the-art.

Overall, our contributions are summarized as follows:

\begin{itemize}
    \item We propose a Half-Learning Half-Distillation mechanism that applies soft distillation for old classes and binary-based optimization for new classes to effectively balance retention and acquisition.
    % To address the conflicting optimization targets between old and new classes, we propose the Half Learning Half Distillation classification loss that offers soft distillation for old classes and binary-based optimization for new classes. 
    \item An extra Query Conflict Reduction module is proposed to refine queries for new classes while preserving unrefined features, which enables Importance-based Knowledge Distillation for remembering the key features.
    \item Through extensive quantitative and qualitative evaluations on the ADE20K dataset, we demonstrate the state-of-the-art performance of our model in both Class Incremental Semantic and Panoptic Segmentation tasks.
\end{itemize}






==> sec/2_relatedwork.tex <==
\section{Related Work}
\label{sec:related_work}

%-------------------------------------------------------------------------
\subsection{Semantic and Panoptic Segmentation}\label{sec:ss_ps}

Semantic segmentation aims to classify each pixel in an image, which focuses on the complete coverage of object(s) in each category. 
The pioneering work FCN~\cite{fcn} and U-Net~\cite{unet} introduces a pixel-wise classification paradigm by removing the fully connected layers. Since then, a large number of approaches~\cite{deeplabv1,deeplabv2, deeplabv3,chen2018encoder,object17,segnet17,refinenet17,segmenter21} following the paradigm have been proposed, containing effective modules like ASPP~\cite{deeplabv3} and pyramid structure~\cite{pspnet17}. 
In contrast, panoptic segmentation~\cite{panoptic} combines the goals of both semantic segmentation and instance segmentation, requiring the classification of every pixel while distinguishing different instances of the same category. 
These two tasks have once been addressed separately due to the limitation of the pixel-wise classification paradigm. 
Until recently, the mask classification paradigm~\cite{mask2former,maskformer,der21,mask-trans22} becomes a universal transformer-based architecture capable of solving multiple segmentation tasks all at once. 
MaskFormer~\cite{maskformer} was the first mask classification method combining the class-agnostic mask proposal generation process and mask classification process, enabling both semantic and panoptic segmentation simultaneously. 
Building upon this, Mask2Former~\cite{mask2former} enhanced performance by incorporating multi-scale feature fusion and masked attention techniques. 
% However, in the domains of continual semantic segmentation and continual panoptic segmentation, particularly in mitigating catastrophic forgetting when learning new categories, significant challenges remain unresolved.
However, when it comes to learning additional categories apart from the initial data, mask classification methods still cannot survive the \textit{catastrophic forgetting}. 



%-------------------------------------------------------------------------
\subsection{Continual Segmentation}\label{sec:cs}

% In the context of Class Incremental Learning~(CIL), fine-tuning models on new training data often results in a significant decline in performance on old categories, a phenomenon known as \textit{catastrophic forgetting}~\cite{catastrophic89,catastrophic95,catastrophic99,lifelong98}. 
% Incremental learning has emerged as a solution to this issue, traditionally studied within the realm of image classification tasks~\cite{chaudhry2018efficient,douillard2020podnet,douillard2022dytox,kirkpatrick2017overcoming,rusu2016progressive,yan2021dynamically}. 
In Class Incremental Learning~(CIL), fine-tuning models on new data often results in a significant decline in performance on old categories, known as \textit{catastrophic forgetting}~\cite{catastrophic99,lifelong98}. 
Various studies~\cite{incremental22,plop21,mib20,modeling22,tackling21,recall21,continual21,rbc22} provide solutions to mitigate forgetting, including remembering representative old samples~\cite{recall21,gss19,ccbo20,gradient17,ssul21,saving24,alife22,continual23}, compensation losses~\cite{cs2k24,foundation23,sdr21,ewf23}, and prompt representations~\cite{introducing23,learning22,incre23}. 
The achievements in CIL raise interest in more challenging segmentation tasks. 
% However, there is growing interest in its application to semantic segmentation~\cite{cermelli2020modeling,cha2021ssul,douillard2021plop,michieli2021continual,phan2022class,zhang2022representation,zhao2022rbc}. 
% Pioneering work in this field~\cite{cermelli2020modeling} identified additional challenges posed by incremental segmentation tasks. 
Class Incremental Semantic Segmentation~(CISS) is first introduced in MiB~\cite{mib20}, reconstructing background regions to address \textit{background shifting} that occurs during each incremental step.
% Specifically, during incremental steps, old categories are labeled as background in new training data, leading to the problem of background shift, which exacerbates catastrophic forgetting.
Since then, most methods~\cite{dkd22,rcil22} have employed techniques such as knowledge distillation~\cite{lwf17}, pseudo-labels from old models~\cite{plop21,comformer23}, redefining background class~\cite{mib20,background24} to mitigate \textit{background shifting}. 
%anqi: incremented 是类vit的网络吧，不是mask classification
% Recently, transformer-based approaches like Incrementer~\cite{shang2023incrementer} have reframed semantic segmentation from a pixel-wise classification problem to a mask classification task, leveraging model strengths to achieve better performance. 
% However, prior studies primarily focused on incremental semantic segmentation, with less attention given to the more challenging domain of incremental panoptic segmentation.
However, prior approaches are primarily built upon the pixel-wise classification method, such as DeepLabV3~\cite{deeplabv3}. 
Therefore, CoMFormer~\cite{comformer23} first utilizes the mask classification segmentation model Mask2Former~\cite{mask2former} enabling solving both CISS and Class Incremental Panoptic Segmentation~(CIPS) tasks. 
ECLIPSE~\cite{eclipse24} introduces dynamic model structure expansion methods to extend learnable parameters for new classes and freezes the old parameters. 
CoMasTRe~\cite{comastre24} distill the queries matched to the old queries with high probability on old classes. 
BalConpas~\cite{balconpas24} balance the class proportion on selecting representative replay samples.
\red{These methods, however, often fall into finding the balance point between acquisition and preservation. Our approach deconstructs two objectives by separating queries to mitigate the conflict.}
% Nevertheless, CoMFormer’s indiscriminate distillation approach hampers the model's ability to learn new categories, and ECLIPSE's dynamic expansion results in increased storage and computational costs. In contrast, our method judiciously selects distillation targets and assigns varying distillation weights, ensuring the retention of previous knowledge while maintaining the capability to learn new information, without incurring additional storage overhead due to dynamic model expansion during incremental steps.
%anqi: 视实验结果情况再想一下怎么写最后


%-------------------------------------------------------------------------



==> sec/3_Preliminaries.tex <==
\section{Preliminaries}
\label{sec:preliminaries}

\subsection{Problem Definition}\label{sec:definition}

In continual segmentation, the model is tasked with an incremental learning challenge over $T$ steps.
At each step $t\in\{1, \ldots, T\}$, the model is trained to recognize a unique set of classes $\bm{C}^{t}$, where the intersection across all sets from $i$ to $T$ is empty $\bigcap_{t=1}^{T}\bm{C}^{t}= \varnothing$ and their union forms the complete set of classes $\bigcup_{t=1}^{T}\bm{C}^{t}=\mathcal{\bm{C}}$.
At the current step $t$, the training dataset $\bm{D}_{train}^t$ consists of image-label pairs $(\bm{x}^{t},\bm{y}^{t})$, where $\bm{x}^{t}$ represents an image and $\bm{y}^{t}$ its corresponding segmentation label.
The labels $\bm{y}^{t}$ are available only for the classes $\bm{C}^{t}$ that need to be learned at this step, while labels for previously learned classes $\bm{C}^{1:t-1}$ and future classes $\bm{C}^{t+1:T}$ are inaccessible.
After completing training at this step, the model must perform segmentation across all classes learned up to that point, $\bm{C}^{1:t}$, thereby preventing catastrophic forgetting of the old classes $\bm{C}^{1:t-1}$ while effectively acquiring new ones $\bm{C}^{t}$.

\subsection{Revisiting Mask2Former and Pseudo-Labeling}\label{sec:psd}

The recent advanced universal segmentation network, Mask2Former~\cite{mask2former}, has favored the class incremental semantic and panoptic segmentation~(CISS and CIPS) tasks for its innovative proposal-based structure.
Mask2Former deviates from traditional pixel-wise classification pipelines by introducing a class-agnostic mask prediction and classification mechanism.
Specifically, the backbone $\bm{f}_b$ and the pixel decoder $\bm{f}_p$ generate multi-scale features that interact with $N$ learnable queries through multiple self-attention and cross-attention layers in the transformer decoder $\bm{f}_t$. 
These $N$ output queries $Q\in\mathbb{R}^{C_{Q}\times N}$ undergo further processing through two linear layers to form mask embeddings $\mathcal{E}_{mask}\in \mathbb{R}^{D\times N}$ and class embeddings $\mathcal{E}_{cls} \in\mathbb{R}^{{(C+1)}\times N}$.
The mask embeddings $\mathcal{E}_{mask}$ yield $N$ mask predictions $\bm{M}\in\mathbb{R}^{N\times H\times W}$ via dot product between each mask embedding and per-pixel embeddings $\mathcal{E}_{pixel}\in\mathbb{R}^{D\times H\times W}$ from $\bm{f}_p$, while $\mathcal{E}_{cls}$ accounts for the classification predictions of these masks.
Note that the additional channel in $\mathcal{E}_{cls}$ represents the \textit{no-obj} class, an auxiliary category utilized during training but excluded during inference. 

In the contexts of CISS and CIPS, where ground truth for old classes $\bm{C}^{1:t-1}$ are inaccessible, pseudo-labeling becomes crucial.
PLOP~\cite{plop21} introduces this strategy by generating pixel-level pseudo ground truths for $\bm{C}^{1:t-1}$, adapted to the mask-based structure by  CoMFormer~\cite{comformer23}, the first method based on Mask2Former for CISS and CIPS tasks.
This adaptation involves weighting the mask predictions $\bm{M}$ by the corresponding maximum class embedding score after the softmax process over the $C+1$ dimensions, i.e., $\max_{c=0}^{\lvert \bm{C}^{0:t-1} \rvert}(\text{softmax}_{c=0}^{|\bm{C}^{0:t-1}|}(\mathcal{E}_{cls}))$ to form $\bm{M}_\omega$, with associated categories $C_\omega = \arg\max_{c=0}^{|\bm{C}^{0:t-1}|}\mathcal{E}_{cls} \in \mathbb{R}^{N}$.
The pseudo-labeling process then labels the pixels outside the union of $\bm{y}^t$ with the category $c$ that achieves the maximum score across $\bm{M}_w$ and $\bm{C}_w$: 
\begin{equation}
    \tilde{M}_c(h,w) = 
    \begin{cases}
        1  & 
        \begin{aligned}
            \text{if}\quad c= &C_\omega[{\arg\max}_{n=1}^NM_w(n, h,w)] \\
            &\vee \max_{c\in C^{t}} y^t(h, w)=0, 
        \end{aligned}\\
        0 & \text{else }
    \end{cases}
\end{equation}
where $n$ indexes the $N$ proposals, and $h, w$ are the pixel coordinates.
This pseudo-labeling strategy has become foundational for CISS and CIPS methods~\cite{comformer23}. 

==> sec/4_method.tex <==
\section{Proposed Method}
\label{sec:method}

%-------------------------------------------------------------------------




%-------------------------------------------------------------------------






%-------------------------------------------------------------------------

In our Conflict Mitigation via Branched Optimization~(CoMBO) within the Mask2Former framework, we employ three distinct strategies: 
the \textit{Half-Distillation-Half-Learning Strategy} for targeted knowledge retention, 
\textit{Importance-Based Knowledge Distillation} to prioritize crucial features, 
and \textit{Query Conflict Reduction} for efficient class integration.

\subsection{Query Conflict Reduction}\label{sec:qcr}

As mentioned in Sec.~\ref{sec:psd}, both class embeddings $\mathcal{E}_{cls}$ and mask predictions $\bm{M}$ are generated from the queries $\bm{Q}$. 
% This interface becomes a critical juncture where conflicts between retaining knowledge of old classes and acquiring new classes manifest, which affects both classification and mask qualities, leading to a decline in overall model performance. 
This interface becomes a critical juncture of conflicts between retaining knowledge of old classes and acquiring new classes manifest, which cannot break through the bottleneck of overall performance by simply finding the balance point. 
% The inappropriate learning strategy could simultaneously result in classification and proposal quality reduction. 

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figs/qcr.png}
    \caption{Illustration of the Query Conflict Reduction~(QCR) module. This module refines queries that predict incremental classes, allowing the processes of learning new features and retaining old features to occur separately.
    Note that the QCR module for previous incremental classes is frozen.}
    \label{fig:qcr}
\end{figure}

To deconstruct the crossroad efficiently, we design a Query Conflict Reduction~(QCR) module $f_{QCR}(\cdot)$ as an additional adapter for new classes. 
As shown in Fig.~\ref{fig:qcr}, in most of the scenarios, queries from the previous layer $Q_{l-1}$ have the same classification results as the queries from the current layer due to the similar distribution and the same classification layer, especially in the latter queries. 
Due to the shared classifier and mask generator following different layers of the transformer decoder, the classification results on the same position of queries from adjacent layers are approximately the same.
Thus, we add the adapter for the queries from the penultimate layer $Q_{L-1}$ with classification results of new classes $\bm{C}^{2:t}$, as shown in Fig.~\ref{fig:qcr}. 
To be more specific, the queries $Q_{L-1, \tilde{c}}$ are selected for the adapter of incremental class $\tilde{c} \in \bm{C}^{2:t}$ via:
\begin{equation}
\resizebox{.9\linewidth}{!}{$
    Q_{L-1, \tilde{c}} = \{Q_{L-1}(n), n \in N \wedge \tilde{c}={\arg\max}_{c=0}^{|\bm{C}^{0:t}|}\mathcal{E}_{cls}(n)\},
    $}
\end{equation}
where $Q_{L-1, \tilde{c}}$ could contain none, one, or some selected queries that enable recognizing different instances. 
For each new category, we utilize the corresponding QCR module $f_{QCR,\tilde{c}}(\cdot)$ to refine the group of queries $Q_{L-1, \tilde{c}}$. 
Considering the efficiency and effectiveness, we introduce the low-rank two-layer adaptation as the QCR module: 
\begin{equation}
    \begin{aligned}
         \hat{Q}_{L-1, \tilde{c}} &=  f_{QCR,\tilde{c}}(Q_{L-1, \tilde{c}}) \\
         &=  Q_{L-1, \tilde{c}}W_1W_2 + Q_{L-1, \tilde{c}}, 
    \end{aligned}
\end{equation}
where $\hat{Q}_{L-1, \tilde{c}}$ represent the adapted queries of class $\tilde{c}$, $W_1\in \mathbb{R}^{D\times r}$ and $W_2\in \mathbb{R}^{r\times D}$ denotes the weights for QCR. 
% The rank $r$ satisfies that $r \ll D$ for affordable additional parameters. 
%anqi:  这下面我是想结合mse蒸馏提到如何拆解query的，暂时先留着这个坑
% The QCR module separates the refined queries $\hat{Q}_{L, \tilde{c}}$ relating to new classes from the original queries $Q_{L, \tilde{c}}$, enabling enhancement of $C^t$ from adaptation and keep memorizing the features of $Q_{L, \tilde{c}}$ with IKD in Sec.~\ref{sec:ikd} simultaneously. 
The QCR module separates the refined queries $\hat{Q}_{L, \tilde{c}}$ from the original queries $Q_{L, \tilde{c}}$, enabling a bifurcate structure for simultaneously learning $\bm{C}^t$ with class-specific adaptation and keep memorizing the features of $Q_{L, \tilde{c}}$ as well as the logits of $\bm{C}^{0:t-1}$. 


\subsection{Half-Distillation-Half-Learning Strategy}

Previous approaches based on Mask2Former usually separate the learning and distillation process on class embeddings $\mathcal{E}_{cls}$ due to its different learning strategies compared to pixel-wise segmentation structure~(\textit{e.g.} DeepLabV3), mentioned in Sec.~\ref{sec:psd}. 
This causes conflicts between distillation and learning, where the same logit could have contradictory optimization directions. 
Therefore, it is necessary to unify the optimization process towards a fixed target. 

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/hdhl.png}
    \caption{Details of the Half-Distillation-Half-Learning strategy on $N$ queries, including classification loss on matched queries and Kullback-Leibler Divergence loss on the other queries. The latter involves the logits of both old and current classes. }
    \label{fig:hdhl}
\end{figure}

Our Half-Distillation-Half-Learning~(HDHL) strategy combines the distillation and learning process for $N$ class embeddings $\mathcal{E}_{cls}$, as illustrated in Fig.~\ref{fig:hdhl}. 
We follow the bipartite matching process of Mask2Former and select embeddings $\mathcal{E}_{cls}^{\bm{C}^t}$  matched to labels of current categories $\bm{C}^t$ and $\mathcal{E}_{cls}^{\bm{C}^{1:t-1}}$ matched to pseudo labels of old categories $\bm{C}^{1:t-1}$. 
These embeddings, following the original optimization strategy, are optimized by cross-entropy loss $\mathcal{L}_{cls}$. 
The other unmatched embeddings $\mathcal{E}_{cls}^{\varnothing^t}$ are grouped as the \textit{no-obj} category in the initial step, yet following the original learning strategy will result in \textit{catastrophic forgetting}. 
Besides, using the distillation strategy for the old categories $\bm{C}^{1:t-1}$ with $\mathcal{E}_{cls}^{\varnothing^{t-1}}$  ignores the learning of current categories $\bm{C}^t$, as learning which region does not belong to $\bm{C}^t$ is the same important as learning which does. 
Considering the problems above, we design a strategy to simultaneously optimize the logits of $\bm{C}^{1:t-1}$ and $\bm{C}^t$ with a shared Kullback-Leibler Divergence $\mathcal{L}_{kl}$:
\begin{equation}
% \resizebox{.9\linewidth}{!}{$
    \mathcal{L}_{kl} = \frac{1}{|\mathcal{E}_{cls}^{\varnothing^t}|} \sum\limits_{j=1}^{|\mathcal{E}_{cls}^{\varnothing^t}|} \sum\limits_{c=0}^{|\bm{C}^{0:t}|} \mathcal{\varphi}_{cls}^{\varnothing^{t-1}}(j, c) \log \frac{\mathcal{\varphi}_{cls}^{\varnothing^{t-1}}(j, c)}{\mathcal{\varphi}_{cls}^{\varnothing^t}(j, c)}, 
    % $}
\end{equation}
where 
\begin{equation}
    % \mathcal{\varphi}_{cls}^{\varnothing^t}(j, c) = \frac{\exp(\mathcal{E}_{cls}^{\varnothing^t}(j,c))}{ \sum_{\hat{c}=0}^{|C^{0:t}|}\exp(\mathcal{E}_{cls}^{\varnothing^t}(j,\hat{c}))}, 
    \begin{aligned}
    \mathcal{\varphi}_{cls}^{\varnothing^t}(j, c) &= \mathcal{S}^t(j,c), \\
    \mathcal{\varphi}_{cls}^{\varnothing^{t-1}}(j, c) &= 
        \begin{cases}
          \mathcal{S}^{t-1}(j,c)  & \text{if}\  c\in \bm{C}^{0:t-1}, \\
            0 & \text{else},
        \end{cases}
    \end{aligned}
\end{equation}
and
\begin{equation}
% \resizebox{1.\linewidth}{!}{$
    \mathcal{S}^{t}(j,c) = 
        \frac{\exp(\mathcal{E}_{cls}^{\varnothing^{t}}(j,c))}{ \sum_{\hat{c}=0}^{|\bm{C}^{0:t}|}\exp(\mathcal{E}_{cls}^{\varnothing^{t}}(j,\hat{c}))}
    % $}
\end{equation}
represent the $\mathrm{softmax}$ activation. 

The $\mathcal{L}_{kl}$ not only distill the previous class embedding $\mathcal{E}_{cls}^{\varnothing^{t-1}}$ to the corresponding categories, including the \textit{no-obj} category, but decreasing the logits of current categories to figure out the objects apart from them. 
The unified HDHL strategy maintains the probability distribution of old logits seamlessly with the integration of new logits. 
By combining the original $\mathcal{L}_{cls}$ and the designed $\mathcal{L}_{kl}$ as $\mathcal{L}_{DL}$, the optimization process covers all the class embeddings without contradictory targets: 
\begin{equation}
    \mathcal{L}_{DL} = \lambda_{cls}\cdot \mathcal{L}_{cls} + \lambda_{kl}\cdot \mathcal{L}_{kl}, 
\end{equation}
where $\lambda_{cls}$ and $\lambda_{kl}$ represent the corresponding hyperparameters. 

\subsection{Importance-Based Knowledge Distillation}
\label{sec:ikd}

% To enable the model to learn new categories, fine-tuning on a new dataset is straightforward but often causes catastrophic forgetting due to a lack of old category annotations.
Previous methods mitigate catastrophic forgetting by applying feature distillation, which may hinder the acquisition of new knowledge.
To address this, we propose an Importance-Based Knowledge Distillation~(IKD) method where stronger distillation is applied to features critical for old classes, while less emphasis on features with less pertinent, thus balancing stability with plasticity. 
% This approach is encapsulated in our Importance-Based Knowledge Distillation method (IKD).

% During the label matching stage, output segments are paired with labels from $\bm{y}^{t}$
% using a similarity-based bipartite matching algorithm. 
The importance measurement requires the cost matrix $\mathcal{A} \in \mathbb{R}^{N \times S}$ that is adopted in the bipartite matching process, where $S$ is the number of image labels. 
The values in $\mathcal{A}$ indicate the relationship between queries and classes.
% Analyzing $\mathcal{A}$ helps assess each query's effectiveness in recognizing specific categories.
% This algorithm computes mask and label losses, forming a one-to-one loss matrix $\mathcal{A} \in \mathbb{R}^{N \times S}$, where $N$ is the number of output segments and $S$ is the number of image labels. Analyzing $\mathcal{A}$ helps assess each query's effectiveness in recognizing specific categories.
Specifically, within each image, the transformer decoder outputs $N$ predicted segments, denoted as $\mathcal{Z} = \{(\mathcal{E}_{cls}(n), M(n))\}_{n=1}^{N}$, 
% where $\mathcal{Z}$ represents the outputs segments, 
% $\mathcal{E}_{cls}(n)$ and $\mathcal{E}_{mask}(n)$ denotes the classification prediction and the mask prediction of the $n$\textsuperscript{th} output segment respectively. 
% According to the model's architecture:
% \begin{equation}
%      \mathcal{E}_{cls}(n) = \mathrm{MLP}(f_{l}^{r}(n)),
% \end{equation}
% \begin{equation}
%      \mathcal{E}_{mask}(n) = \mathrm{sigmoid}(\mathrm{MLP}(f_{l}^{r}(n))) \times \mathrm{MLP}(f_{l}^{p})),  
% \end{equation}
% where $l \in [1, L]$ denotes the index of the transformer decoder layers, $f_{l}^{r}$ and $f_{l}^{p}$ denote the output features derived from the $l$-th layers of the transformer decoder and pixel decoder, respectively. MLP denotes a multilayer perceptron, sigmoid is the sigmoid function, and $[\cdot]$ indicates the channel or element index. 
% Based on the obtained $\mathcal{Z}$ from transformer decoder, 
The computation of the cost matrix $\mathcal{A}$ for the output segments $\mathcal{Z}$ in relation to the image labels $\bm{y}^{t} = \{(c_{s}, m_{s})\}_{s=1}^{S}$ is as follows:
\begin{equation}\label{eq:matrix}
\resizebox{.9\linewidth}{!}{$
     \mathcal{A}(n,s) = -\lambda_{cls} \cdot \mathcal{\varphi}_{cls}(n,c_{s}) + \lambda_{mask} \cdot \mathcal{L}_{mask}(\mathcal{E}_{mask}(n),m_{s}),
     $}
\end{equation}
where $\mathcal{\varphi}_{cls}$ represents the result obtained after processing $\mathcal{E}_{cls}$ through the $\text{softmax}(\cdot)$ function, $\lambda_{cls}$ and $\lambda_{mask}$ represent the corresponding hyperparameters.

After each training stage, we compute the cost matrix $\mathcal{A}$ across every image in the training set $\bm{D}^t_{train}$ of the current incremental step $t$. 
The minimum costs among the classes for $N$ segments are accumulated in the corresponding position of buffer $B^t \in \mathbb{R}^{N}$, where segments with lower minimum cost values are more likely to recognize and cover the regions of a class $\bm{C}^t$. 
By normalizing and reversing the values of $B^t$, we derive the importance matrix $I^t_{\bm{C}^t} \in \mathbb{R}^{N}$ of current classes $\bm{C}^t$.
The importance matrix $I^{t+1} \in \mathbb{R}^{N}$ is further estimated via the weighted accumulation of current importance matrix $I^t \in \mathbb{R}^{N}$ and $I^t_{\bm{C}^t}$, where the weights refer to the $|\bm{C}^{1:t-1}|$ and $|\bm{C}^t|$. 
The generated $I^{t+1}$ will be utilized in the next incremental training phase for weighted distillation of the queries $Q^t$, which is computed as follows:
\begin{equation}
     \mathcal{L}_{IKD} = \frac{1}{N}\sum_{n=1}^{N}I^{t}(n) \cdot \|Q^t(n), Q^{t-1}(n)\|_2^2,
\end{equation}
where $\|\cdot\|_2$ denotes the Euclidean distance, $Q^t(n)$ and $Q^{t-1}(n)$ denotes the transformer decoder features from the current model $f^{t}(\cdot)$ and the old model $f^{t-1}(\cdot)$, respectively. 
% $I^{t}(n)$ indicates the importance of a specific query at the $n$\textsuperscript{th} position during the current step.
Algorithm~\ref{algorithm_1} presents the details of the importance estimation procedure after training $f^{t}(\cdot)$.

\begin{algorithm}
\caption{Importance Matrix Estimation}\label{algorithm_1}
\begin{algorithmic}[1]
\STATE \textbf{Input:} current model $f^{t}(\cdot)$, current dataset $\bm{D}^t_{train}$, current importance matrix $I^{t}$
\STATE \textbf{Initialization:} $I^{t+1} \leftarrow 0$ , $B^t \leftarrow 0$ 
\FOR{all $(\bm{x}^{t}, \bm{y}^{t}) \in \bm{D}^t_{train}$}
    \STATE Compute $\mathcal{A}$ following Eq.(\ref{eq:matrix})
    \STATE Update the buffer:
    \STATE $B^t \leftarrow B^t + \min(\mathcal{A}, \mathrm{axis=1})$
\ENDFOR
% \STATE Calculate the importance $I^{t}_{C^t}$ based on $B^t$:
\FOR{$n \in \{1,2,...,N\}$}
    \STATE $I^{t}_{C^t}(n) \leftarrow 1 - \frac{B^t(n) - \mathrm{min}(B^t)}{\mathrm{max}(B^t) - \mathrm{min}(B^t)}$
    % \STATE Weight the importance $I^{t+1}$ based on the number of categories: 
    \STATE $I^{t+1}(n) \leftarrow \frac{|\bm{C}^{1:t-1}|}{|\bm{C}^{1:t}|} \cdot I^{t}(n) + \frac{|\bm{C}^{t}|}{|\bm{C}^{1:t}|} \cdot I^{t}_{\bm{C}^t}(n)$
\ENDFOR
\STATE \textbf{Output:} Importance matrix $I^{t+1}$ for step $t+1$
\end{algorithmic}
\end{algorithm}



\subsection{Objective Function}

Overall, the objective function of CoMBO is as follows:
\begin{equation}
    \mathcal{L}_{H} = \mathcal{L}_{DL} + \lambda_{IKD}\mathcal{L}_{IKD}. 
\end{equation}
CoMBO assists incremental learning of Mask2Former~\cite{mask2former} following its losses on proposals. 

==> sec/5_experiments.tex <==
\begin{table*}[!t]
    \centering
    
    % Subtable 1 for 100-50, 100-10, and 100-5
    % \begin{subtable}{\linewidth}
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{r|ccc|ccc|ccc|ccc}
    \toprule
    \multirow{2}{*}{Method} & \multicolumn{3}{c|}{\textbf{100-50} (2 steps)} & \multicolumn{3}{c|}{\textbf{100-10} (6 steps)} & \multicolumn{3}{c|}{\textbf{100-5} (11 steps)} &  \multicolumn{3}{c}{\textbf{50-50}~(3 steps)}\\
    & 1-100 & 101-150 & all & 1-100 & 101-150 & all & 1-100 & 101-150 & all  & 1-50& 51-150&all\\
    \midrule
    FT & 0.0 & 1.3 & 0.4 & 0.0 & 2.9 & 1.0 & 0.0 & 25.8 & 8.6  & 0.0 & 12.0 &8.1 
\\
    MiB~\cite{mib20}\pub{CVPR20} & 35.1 & 19.3 & 29.8 & 27.1 & 10.0 & 21.4 & 24.0 & 6.5 & 18.1  & 42.4 & 15.5 &24.4 
\\
    PLOP~\cite{plop21}\pub{CVPR21} & 40.2 & 22.4 & 34.3 & 30.5 & 17.5 & 26.1 & 28.1 & 15.7 & 24.0  & 45.8 & 18.7 &27.7 
\\
    % EWF~\cite{ewf23}\pub{CVPR23} & 37.9 & 4.4 & 26.8 & 35.6 & 0.0 & 23.7 & 32.4 & 0.0 & 21.6  & 35.1 & 2.3 &13.2 \\
    CoMFormer~\cite{comformer23}\pub{CVPR23} & 41.1 & \textbf{27.7} & 36.7 & 36.0 & 17.1 & 29.7 & 34.4 & 15.9 & 28.2  & 45.0 & 19.3 &27.9 
\\
    ECLIPSE~\cite{eclipse24}\pub{CVPR24} & 41.7 & 23.5 & 35.6 & 41.4 & 18.8 & 33.9 & 41.1 & 16.6 & \textbf{32.9}  & 46.0 & 20.7 &29.2 
\\
    BalConpas~\cite{balconpas24}\pub{ECCV24} & 42.8 & \underline{25.7} & \underline{37.1} & 40.7 & \underline{22.8} & \underline{34.7} & 36.1 & \underline{20.3} & 30.8  & 51.2 & \underline{26.5} &\underline{34.7} 
\\
    \midrule
    CoMBO~\pub{Ours} & 43.9 & 25.6 & \textbf{37.8} & 40.8 & \textbf{25.2} & \textbf{35.6} & 36.1 & \textbf{20.5} & \underline{30.9}  & 50.7 & \textbf{28.2} &\textbf{35.7} 
\\
    \midrule
    \rowcolor{gray!30}
    Joint & 43.8 & 30.9 & 39.5 & 43.8 & 30.9 & 39.5 & 43.8 & 30.9 & 39.5  & 50.7 & 33.9 &39.5 \\
    \bottomrule
    \end{tabular}
    }
   %  % \caption{}
   %  \end{subtable}
   % \hspace{1mm} 
    
   %  % Subtable 2 for 50-50, 50-10, and 50-20
   %  \begin{subtable}{\linewidth}
   %  \centering
   %  \begin{tabular}{r|ccc|ccc|ccc}
   %  \toprule
   %  \multirow{2}{*}{Method} & \multicolumn{3}{c|}{\textbf{50-50} (3 steps)} & \multicolumn{3}{c|}{\textbf{50-20} (6 steps)} & \multicolumn{3}{c}{\textbf{50-10} (11 steps)} \\
   %  & 1-50 & 51-150 & all & 1-50 & 51-150 & all & 1-50 & 51-150 & all \\
   %  \midrule
   %  FT & 0.0 & 12.0 & 8.1 & 0.0 & 4.4 & 2.9 & 0.0 & 1.7 & 1.1 \\
   %  MiB~\cite{mib20}\pub{CVPR20} & 42.4 & 15.5 & 24.4 & 38.8 & 10.9 & 20.2 & 34.9 & 7.7 & 16.8 \\
   %  PLOP~\cite{plop21}\pub{CVPR21} & 45.8 & 18.7 & 27.7 & 43.9 & 16.2 & 25.4 & 39.9 & 15.0 & 23.3 \\
   %  EWF~\cite{ewf23}\pub{CVPR23} & 35.1 & 2.3 & 13.2 & - & - & - & - & - & - \\
   %  CoMFormer~\cite{comformer23}\pub{CVPR23} & 45.0 & 19.3 & 27.9 & 42.7 & 17.2 & 25.7 & 38.5 & 15.6 & 23.2 \\
   %  ECLIPSE~\cite{eclipse24}\pub{CVPR24} & 46.0 & 20.7 & 29.2 & 46.4 & 19.6 & 28.6 & 45.9 & 17.3 & 26.8 \\
   %  BalConpas~\cite{balconpas24}\pub{ECCV24} & 51.2 & 26.5 & \underline{34.7} & 48.7 & 27.2 & \underline{34.3} &  44.3& 24.3 & \underline{31.0} \\
   %  \midrule
   %  Ours & 51.0 & 28.7 & \textbf{36.1} & 47.5 & 27.9 & \textbf{34.4} & 42.9 & 23.8 & \textbf{30.2} \\
   %  \midrule
   %  \rowcolor{gray!30}
   %  Joint & 50.7 & 33.9 & 39.5 & 50.7 & 33.9 & 39.5 & 50.7 & 33.9 & 39.5 \\
   %  \bottomrule
   %  \end{tabular}
   %  % \caption{}
   %  \end{subtable}
    \caption{Quantitative comparison under Class Incremental Panoptic Segmentation with state-of-the-art exemplar-free methods on ADE20K in PQ. 
    Scores of novel classes and all classes in \textbf{bold} are the best while \underline{underlined} are the second best. }
    \label{tab:ade_ps}
\end{table*}

\section{Experimental Results} \label{sec:exp}

\subsection{Experimental Setup}

\paragraph{Datasets. }
We follow the settings of previous works~\cite{comformer23,eclipse24,balconpas24} and evaluate our approach on the ADE20K~\cite{ade17} dataset.
This dataset is specifically designed to support both panoptic and semantic segmentation tasks.
ADE20K contains 150 classes, including 100 \textit{thing} classes and 50 \textit{stuff} classes. 
The dataset is composed of 20,210 images for training and 2000 images for validation. 

\paragraph{Evaluation Metrics.}
For Weakly Supervised Incremental Semantic Segmentation, we adopt the widely-used mean Intersection over Union~(mIoU) for evaluation. 
The Intersection over Union~(IoU) is calculated as $\text{IoU} = \frac{TP}{TP+FP+FN}$, where $TP$, $FP$, and $FN$ denote the number of true-positive, false-positive, and false-negative pixels in the prediction result, respectively. 
The mIoU metric averages the IoU across all classes for more comprehensive measurement.
For Class Incremental Panoptic Segmentation, we follow the previous methods~\cite{comformer23} and employ Panoptic Quality~(PQ) as the evaluation metric. 
PQ is defined by the product of Recognition Quality~(RQ) and Segmentation Quality~(SQ). 
To measure the incremental ability of the methods, we compute the corresponding metrics for the initial classes $\bm{C}^1$, the incremental classes $\bm{C}^{2:T}$, and the aggregate of all classes $\bm{C}^{1:T}$. 

\paragraph{Protocols.}
We follow the previous incremental protocols and define representative scenarios as $N_{ini}-N_{inc}$, where $N_{ini}$ and $N_{inc}$ respectively denote the quantity of classes in the initial step and each incremental step. 
For example, in $100\text{-}10$ scenario, training process begins with 100 classes, followed by 10 new classes per incremental step without annotations of old classes. 
For both CIPS and CISS, we do evaluations on the following scenarios: $100\text{-}10$ (6 steps), $100\text{-}50$ (2 steps), $100\text{-}5$ (11 steps) and $50\text{-}50$ (3 steps). 

\paragraph{Implementation Details.}
Our approach is based on the structure of Mask2Former~\cite{mask2former}. 
Following previous CISS and CIPS approaches, we utilize ResNet-50~\cite{resnet16} as backbone for CIPS and ResNet-101 for CISS, with both pre-trained on ImageNet~\cite{imagenet}.
The input resolution of the images is $640\times640$ with all-time batch size of 8.
We follow the training hyperparameter of Mask2Former in the initial step, with a learning rate of $10^{-4}$ and iterations of 160,000.
During the incremental steps, we set 1,000 iterations per class with a learning rate of $5\times10^{-5}$. 
% The batch size is set to 8 in both stages.
The coefficients $r$, $\lambda_{cls}$, $\lambda_{kl}$, $\lambda_{IKD}$ are respectively set to 16, 2, 5, 3. 
All experiments are conducted on the NVIDIA RTX 4090. 

\begin{table*}[!t]
    \centering  
    % Subtable 1 for 100-50, 100-10, and 100-5
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{r|ccc|ccc|ccc|ccc}
    \toprule
    \multirow{2}{*}{Method} & \multicolumn{3}{c|}{\textbf{100-50} (2 steps)} & \multicolumn{3}{c|}{\textbf{100-10} (6 steps)} & \multicolumn{3}{c|}{\textbf{100-5} (11 steps)} & \multicolumn{3}{c}{\textbf{50-50} (3 steps)}\\
    & 1-100 & 101-150 & all & 1-100 & 101-150 & all & 1-100 & 101-150 & all  & 1-50& 51-150&all\\
    \midrule
    FT & 0.0 & 26.7 & 8.9 & 0.0 & 2.3 & 0.8 & 0.0 & 1.1 & 0.3  & 0.0& 1.7&1.1\\
    MiB~\cite{mib20}\pub{CVPR20} & 37.0 & 24.1 & 32.6 & 23.5 & 10.6 & 26.6 & 21.0 & 6.1 & 16.1  & 45.6& 21.0&29.3\\
    PLOP~\cite{plop21}\pub{CVPR21} & 44.2 & 26.2 & 38.2 & 34.8 & 15.9 & 28.5 & 39.5 & 13.6 & 30.9  & 54.9& 30.2&38.4\\
    % EWF~\cite{ewf23}\pub{CVPR23} & 49.2 & 23.7 & 40.7 & 48.5 & 17.7 & 38.2 & 46.9 & 14.7 & 36.2  & 50.6& 27.0&34.9\\
    CoMFormer~\cite{comformer23}\pub{CVPR23} & 44.7 & 26.2 & 38.4 & 40.6 & 15.6 & 32.3 & 39.5 & 13.6 & 30.9  & 49.2& 26.6&34.1\\
    CoMasTRe~\cite{comastre24}\pub{CVPR24} & 45.7 & 26.0 & 39.2 & 42.3 & 18.4 & 34.4 & 40.8 & 15.8 & 32.6  & 49.8& 26.6&34.5\\
    ECLIPSE~\cite{eclipse24}\pub{CVPR24} & 45.0 & 21.7 & 37.1 & 43.4 & 17.4 & 34.6 & 43.3 & 16.3 & \underline{34.2}  & -& -&-\\
    BalConpas~\cite{balconpas24}\pub{ECCV24} & 49.9 & \underline{30.1} & \underline{43.3} & 47.3 & \underline{24.2} & \underline{38.6} & 42.1 & \underline{17.2} & 33.8  & 55.8& \underline{33.3} &\underline{40.8}\\
    \midrule
    CoMBO~\pub{Ours} & 50.2 & \textbf{34.4} & \textbf{44.9} & 47.8 & \textbf{27.7} & \textbf{41.1} & 44.6 & \textbf{22.6} & \textbf{37.3}  & 55.3& \textbf{36.9} & \textbf{43.0}\\
    \midrule
    \rowcolor{gray!30}
    Joint & 51.7 & 40.2 & 47.8 & 51.7 & 40.2 & 47.8 & 51.7 & 40.2 & 47.8  & 56.6& 43.5&47.8\\
    \bottomrule
    \end{tabular}  
    }
    \caption{Quantitative comparison under Class Incremental Semantic Segmentation with state-of-the-art exemplar-free methods on ADE20K in mIoU. 
    Scores of novel classes and all classes in \textbf{bold} are the best while \underline{underlined} are the second best. } 
    \label{tab:ade_ss}
\end{table*}

\begin{table}[!t]
    % Subtable 1 for 100-50, 100-10, and 100-5
    \centering
    \begin{tabular}{c|c|c|ccc}
        \toprule
        \multirow{2}{*}{HDHL} & \multirow{2}{*}{IKD} & \multirow{2}{*}{QCR} & \multicolumn{3}{c}{\textbf{100-10} (6 steps)} \\ 
        &                       &                       & 1-100 & 101-150 & all \\ \midrule

        &                       &                       & 36.3  & 23.8    & 32.2  \\ 
        \checkmark&                       &             & 39.4  & 24.2     & 34.3   \\ 
        \checkmark&                       \checkmark&   & 40.0  & 24.6    & 34.9   \\ 
        &     \checkmark       &           \checkmark   & 38.8  & 25.4    & 34.4    \\ 
        \checkmark&           \checkmark&    \checkmark & 40.8  & 25.2    & \textbf{35.6}      \\ 
        \bottomrule
    \end{tabular} 
    \caption{Ablation study of the main components on task 100-10 of CIPS. \red{Baseline in the 1\textsuperscript{st} row uses vanilla losses with pseudo-labeling and does not include the QCR module.}} 
    \label{tab:ade_ablation}
\end{table}

\subsection{Quantitative Results}

\paragraph{Comparisons in Class Incremental Panoptic Segmentation. }
We evaluated our approach alongside current exemplar-free approaches on the ADE20K dataset within the framework of Class Incremental Panoptic Segmentation, as detailed in Tab.~\ref{tab:ade_ps}. 
% Our experiments include 4 incremental scenarios: 100-50, 100-10, 100-5, 50-50, as detailed in Tab.~\ref{tab:ade_ps}. 
The performance of our CoMBO surpasses other methods in most of the scenarios, particularly in the challenging 100-10 sub-task, we achieve 35.6\% PQ with at least 3.4\% of advantage on incremental classes compared to the previous state-of-the-art methods, demonstrating the effectiveness from reducing the conflicts. 
Although our approach still underperforms the state-of-the-art approach ECLIPSE on the 100-5 sub-task due to its strong memorization ability from freezing parameters, the performance on the new classes remains advanced. 
Moreover, in the scenario with fewer initial classes, \textit{i.e.} 50-50 sub-task, we maintain our advantage in learning new categories with 28.2\% PQ for incremental classes and 35.7\% PQ for overall performance, widening the gap with the strong distillation methods. 
% Notably, our approach achieves 37.6\% and 35.6\% PQ for the typical sub-tasks of 100-50 and 100-10, respectively. 
% Besides, many previous methods focus on mitigating catastrophic forgetting by enhancing the PQ of larger-proportion old classes to artificially elevate the overall PQ. 
% In contrast, our approach exhibits superior performance in new classes while maintaining performance in old classes, as seen in scenarios like 50-50 and 50-20 with substantial improvements of ?\% and ?\% for new classes compared to the previous state-of-the-art method. This reflects our motivation to address the conflict between preserving old class memory and learning new classes.


\paragraph{Comparisons in Class Incremental Semantic Segmentation. }
We further extended our evaluation to the semantic segmentation benchmark, comparing our approach against previous methods on the ADE20K dataset, as detailed in Tab.~\ref{tab:ade_ss}.
Our approach consistently outperforms previous methods in all tested scenarios. 
Notably, in the typical 100-10 sub-task, it achieves a mIoU of 41.1\%, offering at least a 3.5\% advantage over previous state-of-the-art for incremental classes.
This highlights our approach's effectiveness in mitigating conflicts.
Moreover, on the most challenging long-term incremental 100-5 sub-task, our approach not only improves performance on old classes by 2.5\% but also achieves a significant 5.4\% increase in mIoU for new classes, maintaining model stability while ensuring adaptability.

==> sec/6_ablations.tex <==
\section{Ablation Study}

\subsection{Component Ablations}\label{sec:ab_com}
In this section, we analyze the components of our proposed framework, which include the Half-Distillation-Half-Learning Strategy, Importance-based Knowledge Distillation, and Query Conflict Reducing module. 
Our experiments focus on the 100-10 scenario in the CIPS, as it provides a moderate number of steps to examine the ability of both acquisition and retention. 
% and effectively illustrates performance under typical conditions. 
We evaluate various combinations of these components separately and present the results in Tab.~\ref{tab:ade_ablation}. 
The baseline method utilizes the vanilla loss with pseudo-labeling. 
Under identical experimental conditions, the HDHL Strategy significantly enhances the overall PQ by 2.1\%, 
% demonstrating its effectiveness in preserving knowledge of old classes and more importantly boosting the performance of novel classes. 
demonstrating its ability to unify logits of new classes into the previous logits distribution without contradictory losses. 
The implementation of IKD has 
% enhanced the model's performance across both old and new classes. 
a remarkably 3.7\% increase in the PQ for old classes, underscoring its effectiveness in boosting the capability to retain the knowledge of old classes. 
Furthermore, combined with the QCR module for branched optimization, CoMBO further enhance the performance on both old and new classes, resulting in 0.8\% and 0.6\% enhancement in PQ, respectively, which breaks the bottleneck of finding the balance point as previous state-of-the-arts. 
Consequently, the overall growth in PQ compared to the baseline reaches 3.4\%. 
The above results demonstrate the effectiveness of our CoMBO method and its related modules, showing a noticeable improvement in reducing the conflict on model structures and losses. 

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{figs/rank.pdf}
    \caption{Ablation study of $r$ in QCR module, including PQ performance (left) and number of Params. (right). }
    \label{fig:rank}
\end{figure}

\begin{figure*}[!t]
    \centering    \includegraphics[width=0.88\linewidth]{figs/qualitative.pdf}
    \caption{Qualitative results of CoMBO comparing to Baseline, Baseline+HDHL on 100-10  CIPS task of ADE20K. }
    \label{fig:qual}
\end{figure*}

\subsection{Ablation Study of QCR}

We validate the effectiveness of QCR with different settings of $r$ shown in Fig.~\ref{fig:rank}. 
Under the estimation of performance enhancement and additional parameters, our QCR module achieves the best result when $r=16$, where the quantity of additional parameters comes to 8.2K per class. 
Considering the total parameter of Mask2Former~\cite{mask2former} is 44.9M with ResNet-50, the additional parameters only reach up to 2\% of original parameters in total, which is 5 times less than per class additional parameters of ECLIPSE~\cite{eclipse24} while having better performance on new classes. 

\begin{table}
    \centering
    \begin{tabular}{cc|cc|c}
    \toprule
         \multicolumn{2}{c|}{$\mathcal{L}_{cls}$} &\multicolumn{2}{c|}{$\mathcal{L}_{kl}$}&   \multirow{2}{*}{PQ}\\
         % \cline{1-4}
         $\mathcal{E}_{cls}^{\bm{C}^t}$ \& $\mathcal{E}_{cls}^{\bm{C}^{1:t-1}}$ & $\mathcal{E}_{cls}^{t, \varnothing}$  & $\bm{C}^{0:t-1}$& $\bm{C}^{t}$&    \\
         \midrule
         $\checkmark$&  $\checkmark$ &  &  &  32.2\\
         $\checkmark$&  $\checkmark$ &  $\checkmark$&  &  32.6\\
         $\checkmark$&   &  $\checkmark$&  &  32.2\\
        $\checkmark$& $\checkmark$& $\checkmark$& & 33.5\\
        $\checkmark$&  & $\checkmark$& $\checkmark$& \textbf{34.3}\\
        \bottomrule
    \end{tabular}
    \caption{Ablation study of the HDHL strategy on task 100-10 of CIPS. The 1\textsuperscript{st} row represents the vanilla loss with pseudo-labeling. The last row represents our $\mathcal{L}_{DL}$.}
    \label{tab:hdhl}
\end{table}


\subsection{Ablation Study of HDHL Strategy }

To validate the effectiveness of our Half-Distillation-Half-Learning strategy, we conduct a series of experiments among other strategies, as shown in Tab.~\ref{tab:hdhl}. 
The 1\textsuperscript{st} row with $\mathcal{L}_{cls}$ on all classification embeddings represents the vanilla loss with pseudo-labeling, which is adopted in \cite{comformer23}. 
The 2\textsuperscript{nd} row utilizes an auxiliary distillation on the embeddings following~\cite{comastre24}. Compared to these strategies with tough supervision on unmatched embeddings $\mathcal{E}_{cls}^{t, \varnothing}$ and mostly conflicting losses, our HDHL strategy with soft and concentrated supervision has a better PQ of 34.3. 
Besides, the HDHL design of $\mathcal{L}_{kl}$ ensures the integrity while optimizing the unmatched embeddings $\mathcal{E}_{cls}^{t, \varnothing}$, with improvement of 2.1\% compared to distillation-only strategy in the 3\textsuperscript{rd} row and 0.8\% compared to the simple combination of distillation and $\mathcal{L}_{cls}$. 
The results above show that our HDHL strategy outperforms other learning or distillation strategies on the class embeddings. 


\subsection{Qualitative Analysis}

We conduct the qualitative analysis by comparing our proposed CoMBO to the \textit{Baseline}~(1\textsuperscript{st} row of Tab.~\ref{tab:ade_ablation} and \textit{Baseline+HDHL}~(2\textsuperscript{nd} row of Tab.~\ref{tab:ade_ablation}). 
% In the 1\textsuperscript{st} column, the Baseline method fails to recognize the \textit{screen door}, while the Baseline+HDHL has decreased quality on predicting the initial class \textit{wall}
In the 1\textsuperscript{st}, 2\textsuperscript{nd}, and 5\textsuperscript{th} column, our CoMBO can indicate the incremental classes, \textit{i.e.}, \textit{screen door}, \textit{fountain}, and \textit{ottoman}, while the other methods fail to recognize all of these objects. 
In the 3\textsuperscript{rd} column, our method successfully remembers the \textit{car} in the left instead of covering the object with the prediction of the incremental class \textit{van}. 
Furthermore, our method allows more precise mask prediction of new class \textit{Traffic Light} in the 4\textsuperscript{th} column, demonstrating the effectiveness of refinements on the queries corresponding to new classes. 

==> sec/7_conclusion.tex <==
\section{Conclusion}
In this paper, we present CoMBO, a novel CIS method for mitigating the conflict for balancing the acquisition and retention losses. 
% specifically designed to reduce the conflicts between acquiring new classes and retaining old classes. 
% By reducing the conflict between the optimization objectives for both old and new classes, our method preserves previously learned information while effectively to new class information. 
Our QCR module branches the conflicting optimization target via lightweight class-specific adaptation on queries, enabling the coexistence of learning and distillation on separated queries. 
The HDHL strategy and IKD further reduce the contradictory optimization on classification logits and queries with unified targets, respectively. 
Extensive experimental validation on the ADE20K dataset underscores the superiority of our approach, demonstrating the effectiveness of each component in the CIS task, particularly excelling in performance on new classes.
% Moreover, our method surpasses previous state-of-the-art approaches in most sub-tasks, particularly excelling in performance on new classes.
